FastSample: Accelerating Distributed Graph Neural Network Training for Billion-Scale Graphs

Training Graph Neural Networks(GNNs) on a large monolithic graph presents unique challenges as the graph cannot fit within a single machine and it cannot be decomposed into smaller disconnected components. Distributed sampling-based training distributes the graph across multiple machines and trains the GNN on small parts of the graph that are randomly sampled every training iteration. We show that in a distributed environment, the sampling overhead is a significant component of the training time for large-scale graphs. We propose FastSample which is composed of two synergistic techniques that greatly reduce the distributed sampling time: 1)a new graph partitioning method that eliminates most of the communication rounds in distributed sampling , 2)a novel highly optimized sampling kernel that reduces memory movement during sampling. We test FastSample on large-scale graph benchmarks and show that FastSample speeds up distributed sampling-based GNN training by up to 2x with no loss in accuracy.

==> juans_def.tex <==

% %Always used
% \def \defQfunction 
%         {Q(u):=(1/\sqrt{2\pi})\int_u^\infty e^{-u^2/2} du}
% \def \intinfty  { \int_{-\infty}^{\infty} }
\def\bal#1\eal{\begin{align}#1\end{align}}
\def \var {\text{var}}
\def \bbWn {{\bbW_n}}
\def \bbHn {{\bbH_n}}
\def \deq {\stackrel{d}{=} }
\def \hdag {{\bbh^{f^\dagger g^\dagger}_{l^\dagger}}}
\def \AW {{A_{\bbW}}}
\def \Ah {{A_{h}}}
\def \AX {{A_{X}}}
\def \Anrho {{A_{\nabla \rho}}}
\def \Al {{A_{\ell}}}
\def \Agl {{A_{\nabla\ell}}}
\def \AY {{A_{Y}}}
\def \AnWNN {{A_{\nabla\Phi}}}
\newcommand{\minimize}{\operatornamewithlimits{minimize}}
\newcommand{\non}{\rho}

\newcommand{\lipGrad}{L_\nabla}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Overline
%
\def \ovP {\overline{P}}
\def \ovl {\overline{l}}
\def \ovbbl {\overline{\bbl}}
\def \ovX {\overline{X}}
\def \ovbbX {\overline{\bbX}}
\def \ovp {\overline{p}}
\def \ovbbp {\overline{\bbp}}
\def \ovr {\overline{r}}
\def \ova {\overline{a}}
\def \ovc {\overline{c}}
\def \ovalpha {\overline{\alpha}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Underline
%
\def \undP {\underline{P}}
\def \undl {\underline{l}}
\def \undbbl {\underline{\bbl}}
\def \undX {\underline{X}}
\def \undbbX {\underline{\bbX}}
\def \undp {\underline{p}}
\def \undbbp {\underline{\bbp}}
\def \undr {\underline{r}}
\def \unda {\underline{a}}
\def \undc {\underline{c}}
\def \undalpha {\underline{\alpha}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Overline and Underline
%
\def \undovP     {\underline{\ovP}}
\def \undovX     {\underline{\ovX}}
\def \undovbbX   {\underline{\ovbbX}}
\def \undovp     {\underline{\ovp}}
\def \undovbbp   {\underline{\ovbbp}}
\def \undovr     {\underline{\ovr}}
\def \undova     {\underline{\ova}}
\def \undovc     {\underline{\ovc}}
\def \undovalpha {\underline{\ovalpha}}

%roman symbols
\def \SNR     {\text{\normalfont SNR}   }
\def \ap      {\text{\normalfont ap}   }
\def \best    {\text{\normalfont best} }
\def \Co      {\text{\normalfont Co}   }
\def \Cov     {\text{\normalfont Cov}  }
\def \cov     {\text{\normalfont cov}  }
\def \dest    {\text{\normalfont dest} }
\def \diag    {\text{\normalfont diag} }
\def \eig     {\text{\normalfont eig}  }
\def \for     {\text{\normalfont for}  }
\def \forall  {\text{\normalfont for all}  }
\def \forsome {\text{\normalfont for some}  }
\def \ML      {\text{\normalfont ML}   }
\def \MLE     {\text{\normalfont MLE}  }
\def \ml      {\text{\normalfont ml}   }
\def \mse     {\text{\normalfont mse}  }
\def \rank    {\text{\normalfont rank} }
\def \sign    {\text{\normalfont sign} }
\def \tr      {\text{\normalfont tr}   }

%units
\def \dB      {\, \text{\normalfont dB} }
\def \ms      {\, \text{\normalfont m}/ \text{\normalfont s}}
\def \kmh     {\, \text{\normalfont km}/ \text{\normalfont h}}
\def \m       {\, \text{\normalfont m} }
\def \s       {\, \text{\normalfont s} }
\def \sec     {\, \text{\normalfont sec.} }
\def \msec    {\, \text{\normalfont msec.} }
\def \cm      {\, \text{\normalfont cm} }
\def \km      {\, \text{\normalfont km} }
\def \GHz     {\, \text{\normalfont GHz} }
\def \Hz      {\, \text{\normalfont Hz} }
\def \MHZ     {\, \text{\normalfont MHz} }
\def \kHZ     {\, \text{\normalfont kHz} }


%Probability operators
\newcommand   \E     [1] {{\mathbb E}\left[#1\right]}
\newcommand   \Ec    [1] {{\mathbb E}\left(#1\right)}
\newcommand   \ind   [1] {{\mathbb I \left\{#1\right\}  } }
\renewcommand \Pr    [1] {\text{\normalfont Pr}  \left[#1\right]}
\newcommand   \Prc   [1] {\text{\normalfont Pr}  \left(#1\right)}
\renewcommand \P     [1] {\text{\normalfont P}   \left[#1\right]}
\newcommand   \Pc    [1] {\text{\normalfont P}   \left(#1\right)}
\newcommand   \Pcbig [1] {\text{\normalfont P}   \big(#1 \big)}
\newcommand   \PcBig [1] {\text{\normalfont P}   \Big(#1 \Big)}
% \newcommand   \var   [1] {\text{\normalfont var} \left[#1\right]}
\newcommand   \varc  [1] {\text{\normalfont var} \left(#1\right)}
\renewcommand \Re    [1] {\text{\normalfont Re} \left(#1\right)}
\renewcommand \Im    [1] {\text{\normalfont Im} \left(#1\right)}
\newcommand   \der         [2] {\frac{\partial#1}{\partial#2}}
\newcommand   \inlineder   [2] {\partial#1/\partial#2}


%miscellaneous
\def \naturals {{\mathbb N}}
\def \reals    {{\mathbb R}}
\def \blog { {\bf \log   } }
\def \given{ {\,\big|\,  } }
\newcommand{\st}{\operatornamewithlimits{s.t.}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bar version
%capital alphabet
\def\bbarA{{\ensuremath{\bar A}}}
\def\bbarB{{\ensuremath{\bar B}}}
\def\bbarC{{\ensuremath{\bar C}}}
\def\bbarD{{\ensuremath{\bar D}}}
\def\bbarE{{\ensuremath{\bar E}}}
\def\bbarF{{\ensuremath{\bar F}}}
\def\bbarG{{\ensuremath{\bar G}}}
\def\bbarH{{\ensuremath{\bar H}}}
\def\bbarI{{\ensuremath{\bar I}}}
\def\bbarJ{{\ensuremath{\bar J}}}
\def\bbarK{{\ensuremath{\bar K}}}
\def\bbarL{{\ensuremath{\bar L}}}
\def\bbarM{{\ensuremath{\bar M}}}
\def\bbarN{{\ensuremath{\bar N}}}
\def\bbarO{{\ensuremath{\bar O}}}
\def\bbarP{{\ensuremath{\bar P}}}
\def\bbarQ{{\ensuremath{\bar Q}}}
\def\bbarR{{\ensuremath{\bar R}}}
\def\bbarW{{\ensuremath{\bar W}}}
\def\bbarU{{\ensuremath{\bar U}}}
\def\bbarV{{\ensuremath{\bar V}}}
\def\bbarS{{\ensuremath{\bar S}}}
\def\bbarT{{\ensuremath{\bar T}}}
\def\bbarX{{\ensuremath{\bar X}}}
\def\bbarY{{\ensuremath{\bar Y}}}
\def\bbarZ{{\ensuremath{\bar Z}}}
%lower case alphabet
\def\bbara{{\ensuremath{\bar a}}}
\def\bbarb{{\ensuremath{\bar b}}}
\def\bbarc{{\ensuremath{\bar c}}}
\def\bbard{{\ensuremath{\bar d}}}
\def\bbare{{\ensuremath{\bar e}}}
\def\bbarf{{\ensuremath{\bar f}}}
\def\bbarg{{\ensuremath{\bar g}}}
\def\bbarh{{\ensuremath{\bar h}}}
\def\bbari{{\ensuremath{\bar i}}}
\def\bbarj{{\ensuremath{\bar j}}}
\def\bbark{{\ensuremath{\bar k}}}
\def\bbarl{{\ensuremath{\bar l}}}
\def\bbarm{{\ensuremath{\bar m}}}
\def\bbarn{{\ensuremath{\bar n}}}
\def\bbaro{{\ensuremath{\bar o}}}
\def\bbarp{{\ensuremath{\bar p}}}
\def\bbarq{{\ensuremath{\bar q}}}
\def\bbarr{{\ensuremath{\bar r}}}
\def\bbarw{{\ensuremath{\bar w}}}
\def\bbaru{{\ensuremath{\bar u}}}
\def\bbarv{{\ensuremath{\bar v}}}
\def\bbars{{\ensuremath{\bar s}}}
\def\bbart{{\ensuremath{\bar t}}}
\def\bbarx{{\ensuremath{\bar x}}}
\def\bbary{{\ensuremath{\bar y}}}
\def\bbarz{{\ensuremath{\bar z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of bar version

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   B   L   A   C   K   B   O   A   R   D         B   O   L   D   %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mbA{{\ensuremath{\mathbb A}}}
\def\mbB{{\ensuremath{\mathbb B}}}
\def\mbC{{\ensuremath{\mathbb C}}}
\def\mbD{{\ensuremath{\mathbb D}}}
\def\mbE{{\ensuremath{\mathbb E}}}
\def\mbF{{\ensuremath{\mathbb F}}}
\def\mbG{{\ensuremath{\mathbb G}}}
\def\mbH{{\ensuremath{\mathbb H}}}
\def\mbI{{\ensuremath{\mathbb I}}}
\def\mbJ{{\ensuremath{\mathbb J}}}
\def\mbK{{\ensuremath{\mathbb K}}}
\def\mbL{{\ensuremath{\mathbb L}}}
\def\mbM{{\ensuremath{\mathbb M}}}
\def\mbN{{\ensuremath{\mathbb N}}}
\def\mbO{{\ensuremath{\mathbb O}}}
\def\mbP{{\ensuremath{\mathbb P}}}
\def\mbQ{{\ensuremath{\mathbb Q}}}
\def\mbR{{\ensuremath{\mathbb R}}}
\def\mbS{{\ensuremath{\mathbb S}}}
\def\mbT{{\ensuremath{\mathbb T}}}
\def\mbU{{\ensuremath{\mathbb U}}}
\def\mbV{{\ensuremath{\mathbb V}}}
\def\mbW{{\ensuremath{\mathbb W}}}
\def\mbX{{\ensuremath{\mathbb X}}}
\def\mbY{{\ensuremath{\mathbb Y}}}
\def\mbZ{{\ensuremath{\mathbb Z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   C   A   L   I   G   R   A   P   H   I   C   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ccalA{{\ensuremath{\mathcal A}}}
\def\ccalB{{\ensuremath{\mathcal B}}}
\def\ccalC{{\ensuremath{\mathcal C}}}
\def\ccalD{{\ensuremath{\mathcal D}}}
\def\ccalE{{\ensuremath{\mathcal E}}}
\def\ccalF{{\ensuremath{\mathcal F}}}
\def\ccalG{{\ensuremath{\mathcal G}}}
\def\ccalH{{\ensuremath{\mathcal H}}}
\def\ccalI{{\ensuremath{\mathcal I}}}
\def\ccalJ{{\ensuremath{\mathcal J}}}
\def\ccalK{{\ensuremath{\mathcal K}}}
\def\ccalL{{\ensuremath{\mathcal L}}}
\def\ccalM{{\ensuremath{\mathcal M}}}
\def\ccalN{{\ensuremath{\mathcal N}}}
\def\ccalO{{\ensuremath{\mathcal O}}}
\def\ccalP{{\ensuremath{\mathcal P}}}
\def\ccalQ{{\ensuremath{\mathcal Q}}}
\def\ccalR{{\ensuremath{\mathcal R}}}
\def\ccalW{{\ensuremath{\mathcal W}}}
\def\ccalU{{\ensuremath{\mathcal U}}}
\def\ccalV{{\ensuremath{\mathcal V}}}
\def\ccalS{{\ensuremath{\mathcal S}}}
\def\ccalT{{\ensuremath{\mathcal T}}}
\def\ccalX{{\ensuremath{\mathcal X}}}
\def\ccalY{{\ensuremath{\mathcal Y}}}
\def\ccalZ{{\ensuremath{\mathcal Z}}}
%lower case alphabet
\def\ccala{{\ensuremath{\mathcal a}}}
\def\ccalb{{\ensuremath{\mathcal b}}}
\def\ccalc{{\ensuremath{\mathcal c}}}
\def\ccald{{\ensuremath{\mathcal d}}}
\def\ccale{{\ensuremath{\mathcal e}}}
\def\ccalf{{\ensuremath{\mathcal f}}}
\def\ccalg{{\ensuremath{\mathcal g}}}
\def\ccalh{{\ensuremath{\mathcal h}}}
\def\ccali{{\ensuremath{\mathcal i}}}
\def\ccalj{{\ensuremath{\mathcal j}}}
\def\ccalk{{\ensuremath{\mathcal k}}}
\def\ccall{{\ensuremath{\mathcal l}}}
\def\ccalm{{\ensuremath{\mathcal m}}}
\def\ccaln{{\ensuremath{\mathcal n}}}
\def\ccalo{{\ensuremath{\mathcal o}}}
\def\ccalp{{\ensuremath{\mathcal p}}}
\def\ccalq{{\ensuremath{\mathcal q}}}
\def\ccalr{{\ensuremath{\mathcal r}}}
\def\ccalw{{\ensuremath{\mathcal w}}}
\def\ccalu{{\ensuremath{\mathcal u}}}
\def\ccalv{{\ensuremath{\mathcal v}}}
\def\ccals{{\ensuremath{\mathcal s}}}
\def\ccalt{{\ensuremath{\mathcal t}}}
\def\ccalx{{\ensuremath{\mathcal x}}}
\def\ccaly{{\ensuremath{\mathcal y}}}
\def\ccalz{{\ensuremath{\mathcal z}}}
\def\ccal0{{\ensuremath{\mathcal 0}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of caligraph version
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%hat version
%capital alphabet
\def\hhatA{{\ensuremath{\hat A}}}
\def\hhatB{{\ensuremath{\hat B}}}
\def\hhatC{{\ensuremath{\hat C}}}
\def\hhatD{{\ensuremath{\hat D}}}
\def\hhatE{{\ensuremath{\hat E}}}
\def\hhatF{{\ensuremath{\hat F}}}
\def\hhatG{{\ensuremath{\hat G}}}
\def\hhatH{{\ensuremath{\hat H}}}
\def\hhatI{{\ensuremath{\hat I}}}
\def\hhatJ{{\ensuremath{\hat J}}}
\def\hhatK{{\ensuremath{\hat K}}}
\def\hhatL{{\ensuremath{\hat L}}}
\def\hhatM{{\ensuremath{\hat M}}}
\def\hhatN{{\ensuremath{\hat N}}}
\def\hhatO{{\ensuremath{\hat O}}}
\def\hhatP{{\ensuremath{\hat P}}}
\def\hhatQ{{\ensuremath{\hat Q}}}
\def\hhatR{{\ensuremath{\hat R}}}
\def\hhatW{{\ensuremath{\hat W}}}
\def\hhatU{{\ensuremath{\hat U}}}
\def\hhatV{{\ensuremath{\hat V}}}
\def\hhatS{{\ensuremath{\hat S}}}
\def\hhatT{{\ensuremath{\hat T}}}
\def\hhatX{{\ensuremath{\hat X}}}
\def\hhatY{{\ensuremath{\hat Y}}}
\def\hhatZ{{\ensuremath{\hat Z}}}
%lower case alphabet
\def\hhata{{\ensuremath{\hat a}}}
\def\hhatb{{\ensuremath{\hat b}}}
\def\hhatc{{\ensuremath{\hat c}}}
\def\hhatd{{\ensuremath{\hat d}}}
\def\hhate{{\ensuremath{\hat e}}}
\def\hhatf{{\ensuremath{\hat f}}}
\def\hhatg{{\ensuremath{\hat g}}}
\def\hhath{{\ensuremath{\hat h}}}
\def\hhati{{\ensuremath{\hat i}}}
\def\hhatj{{\ensuremath{\hat j}}}
\def\hhatk{{\ensuremath{\hat k}}}
\def\hhatl{{\ensuremath{\hat l}}}
\def\hhatm{{\ensuremath{\hat m}}}
\def\hhatn{{\ensuremath{\hat n}}}
\def\hhato{{\ensuremath{\hat o}}}
\def\hhatp{{\ensuremath{\hat p}}}
\def\hhatq{{\ensuremath{\hat q}}}
\def\hhatr{{\ensuremath{\hat r}}}
\def\hhatw{{\ensuremath{\hat w}}}
\def\hhatu{{\ensuremath{\hat u}}}
\def\hhatv{{\ensuremath{\hat v}}}
\def\hhats{{\ensuremath{\hat s}}}
\def\hhatt{{\ensuremath{\hat t}}}
\def\hhatx{{\ensuremath{\hat x}}}
\def\hhaty{{\ensuremath{\hat y}}}
\def\hhatz{{\ensuremath{\hat z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of hat version
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tilde version
%capital alphabet
\def\tdA{{\ensuremath{\tilde A}}}
\def\tdB{{\ensuremath{\tilde B}}}
\def\tdC{{\ensuremath{\tilde C}}}
\def\tdD{{\ensuremath{\tilde D}}}
\def\tdE{{\ensuremath{\tilde E}}}
\def\tdF{{\ensuremath{\tilde F}}}
\def\tdG{{\ensuremath{\tilde G}}}
\def\tdH{{\ensuremath{\tilde H}}}
\def\tdI{{\ensuremath{\tilde I}}}
\def\tdJ{{\ensuremath{\tilde J}}}
\def\tdK{{\ensuremath{\tilde K}}}
\def\tdL{{\ensuremath{\tilde L}}}
\def\tdM{{\ensuremath{\tilde M}}}
\def\tdN{{\ensuremath{\tilde N}}}
\def\tdO{{\ensuremath{\tilde O}}}
\def\tdP{{\ensuremath{\tilde P}}}
\def\tdQ{{\ensuremath{\tilde Q}}}
\def\tdR{{\ensuremath{\tilde R}}}
\def\tdW{{\ensuremath{\tilde W}}}
\def\tdU{{\ensuremath{\tilde U}}}
\def\tdV{{\ensuremath{\tilde V}}}
\def\tdS{{\ensuremath{\tilde S}}}
\def\tdT{{\ensuremath{\tilde T}}}
\def\tdX{{\ensuremath{\tilde X}}}
\def\tdY{{\ensuremath{\tilde Y}}}
\def\tdZ{{\ensuremath{\tilde Z}}}
%lower case alphabet
\def\tda{{\ensuremath{\tilde a}}}
\def\tdb{{\ensuremath{\tilde b}}}
\def\tdc{{\ensuremath{\tilde c}}}
\def\tdd{{\ensuremath{\tilde d}}}
\def\tde{{\ensuremath{\tilde e}}}
\def\tdf{{\ensuremath{\tilde f}}}
\def\tdg{{\ensuremath{\tilde g}}}
\def\tdh{{\ensuremath{\tilde h}}}
\def\tdi{{\ensuremath{\tilde i}}}
\def\tdj{{\ensuremath{\tilde j}}}
\def\tdk{{\ensuremath{\tilde k}}}
\def\tdl{{\ensuremath{\tilde l}}}
\def\tdm{{\ensuremath{\tilde m}}}
\def\tdn{{\ensuremath{\tilde n}}}
\def\tdo{{\ensuremath{\tilde o}}}
\def\tdp{{\ensuremath{\tilde p}}}
\def\tdq{{\ensuremath{\tilde q}}}
\def\tdr{{\ensuremath{\tilde r}}}
\def\tdw{{\ensuremath{\tilde w}}}
\def\tdu{{\ensuremath{\tilde u}}}
\def\tdv{{\ensuremath{\tilde r}}}
\def\tds{{\ensuremath{\tilde s}}}
\def\tdt{{\ensuremath{\tilde t}}}
\def\tdx{{\ensuremath{\tilde x}}}
\def\tdy{{\ensuremath{\tilde y}}}
\def\tdz{{\ensuremath{\tilde z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of tilde version
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%check version
%lower case alphabet
\def\chka{{\ensuremath{\check a}}}
\def\chkb{{\ensuremath{\check b}}}
\def\chkc{{\ensuremath{\check c}}}
\def\chkd{{\ensuremath{\check d}}}
\def\chke{{\ensuremath{\check e}}}
\def\chkf{{\ensuremath{\check f}}}
\def\chkg{{\ensuremath{\check g}}}
\def\chkh{{\ensuremath{\check h}}}
\def\chki{{\ensuremath{\check i}}}
\def\chkj{{\ensuremath{\check j}}}
\def\chkk{{\ensuremath{\check k}}}
\def\chkl{{\ensuremath{\check l}}}
\def\chkm{{\ensuremath{\check m}}}
\def\chkn{{\ensuremath{\check n}}}
\def\chko{{\ensuremath{\check o}}}
\def\chkp{{\ensuremath{\check p}}}
\def\chkq{{\ensuremath{\check q}}}
\def\chkr{{\ensuremath{\check r}}}
\def\chkw{{\ensuremath{\check w}}}
\def\chku{{\ensuremath{\check u}}}
\def\chkv{{\ensuremath{\check v}}}
\def\chks{{\ensuremath{\check s}}}
\def\chkt{{\ensuremath{\check t}}}
\def\chkx{{\ensuremath{\check x}}}
\def\chky{{\ensuremath{\check y}}}
\def\chkz{{\ensuremath{\check z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of check version
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Bold version
% upper case bold
\def\bbone{{\ensuremath{\mathbf 1}}}
\def\bbzero{{\ensuremath{\mathbf 0}}}
\def\bbA{{\ensuremath{\mathbf A}}}
\def\bbB{{\ensuremath{\mathbf B}}}
\def\bbC{{\ensuremath{\mathbf C}}}
\def\bbD{{\ensuremath{\mathbf D}}}
\def\bbE{{\ensuremath{\mathbf E}}}
\def\bbF{{\ensuremath{\mathbf F}}}
\def\bbG{{\ensuremath{\mathbf G}}}
\def\bbH{{\ensuremath{\mathbf H}}}
\def\bbI{{\ensuremath{\mathbf I}}}
\def\bbJ{{\ensuremath{\mathbf J}}}
\def\bbK{{\ensuremath{\mathbf K}}}
\def\bbL{{\ensuremath{\mathbf L}}}
\def\bbM{{\ensuremath{\mathbf M}}}
\def\bbN{{\ensuremath{\mathbf N}}}
\def\bbO{{\ensuremath{\mathbf O}}}
\def\bbP{{\ensuremath{\mathbf P}}}
\def\bbQ{{\ensuremath{\mathbf Q}}}
\def\bbR{{\ensuremath{\mathbf R}}}
\def\bbW{{\ensuremath{\mathbf W}}}
\def\bbU{{\ensuremath{\mathbf U}}}
\def\bbV{{\ensuremath{\mathbf V}}}
\def\bbS{{\ensuremath{\mathbf S}}}
\def\bbT{{\ensuremath{\mathbf T}}}
\def\bbX{{\ensuremath{\mathbf X}}}
\def\bbY{{\ensuremath{\mathbf Y}}}
\def\bbZ{{\ensuremath{\mathbf Z}}}
%lower case bold
\def\bba{{\ensuremath{\mathbf a}}}
\def\bbb{{\ensuremath{\mathbf b}}}
\def\bbc{{\ensuremath{\mathbf c}}}
\def\bbd{{\ensuremath{\mathbf d}}}
\def\bbe{{\ensuremath{\mathbf e}}}
\def\bbf{{\ensuremath{\mathbf f}}}
\def\bbg{{\ensuremath{\mathbf g}}}
\def\bbh{{\ensuremath{\mathbf h}}}
\def\bbi{{\ensuremath{\mathbf i}}}
\def\bbj{{\ensuremath{\mathbf j}}}
\def\bbk{{\ensuremath{\mathbf k}}}
\def\bbl{{\ensuremath{\mathbf l}}}
\def\bbm{{\ensuremath{\mathbf m}}}
\def\bbn{{\ensuremath{\mathbf n}}}
\def\bbo{{\ensuremath{\mathbf o}}}
\def\bbp{{\ensuremath{\mathbf p}}}
\def\bbq{{\ensuremath{\mathbf q}}}
\def\bbr{{\ensuremath{\mathbf r}}}
\def\bbw{{\ensuremath{\mathbf w}}}
\def\bbu{{\ensuremath{\mathbf u}}}
\def\bbv{{\ensuremath{\mathbf v}}}
\def\bbs{{\ensuremath{\mathbf s}}}
\def\bbt{{\ensuremath{\mathbf t}}}
\def\bbx{{\ensuremath{\mathbf x}}}
\def\bby{{\ensuremath{\mathbf y}}}
\def\bbz{{\ensuremath{\mathbf z}}}
\def\bb0{{\ensuremath{\mathbf 0}}}
%

% roman 
\def\rmA{{\ensuremath\text{A}}}
\def\rmB{{\ensuremath\text{B}}}
\def\rmC{{\ensuremath\text{C}}}
\def\rmD{{\ensuremath\text{D}}}
\def\rmE{{\ensuremath\text{E}}}
\def\rmF{{\ensuremath\text{F}}}
\def\rmG{{\ensuremath\text{G}}}
\def\rmH{{\ensuremath\text{H}}}
\def\rmI{{\ensuremath\text{I}}}
\def\rmJ{{\ensuremath\text{J}}}
\def\rmK{{\ensuremath\text{K}}}
\def\rmL{{\ensuremath\text{L}}}
\def\rmM{{\ensuremath\text{M}}}
\def\rmN{{\ensuremath\text{N}}}
\def\rmO{{\ensuremath\text{O}}}
\def\rmP{{\ensuremath\text{P}}}
\def\rmQ{{\ensuremath\text{Q}}}
\def\rmR{{\ensuremath\text{R}}}
\def\rmW{{\ensuremath\text{W}}}
\def\rmU{{\ensuremath\text{U}}}
\def\rmV{{\ensuremath\text{V}}}
\def\rmS{{\ensuremath\text{S}}}
\def\rmT{{\ensuremath\text{T}}}
\def\rmX{{\ensuremath\text{X}}}
\def\rmY{{\ensuremath\text{Y}}}
\def\rmZ{{\ensuremath\text{Z}}}
%lower case bold
\def\rma{{\ensuremath\text{a}}}
\def\rmb{{\ensuremath\text{b}}}
\def\rmc{{\ensuremath\text{c}}}
\def\rmd{{\ensuremath\text{d}}}
\def\rme{{\ensuremath\text{e}}}
\def\rmf{{\ensuremath\text{f}}}
\def\rmg{{\ensuremath\text{g}}}
\def\rmh{{\ensuremath\text{h}}}
\def\rmi{{\ensuremath\text{i}}}
\def\rmj{{\ensuremath\text{j}}}
\def\rmk{{\ensuremath\text{k}}}
\def\rml{{\ensuremath\text{l}}}
\def\rmm{{\ensuremath\text{m}}}
\def\rmn{{\ensuremath\text{n}}}
\def\rmo{{\ensuremath\text{o}}}
\def\rmp{{\ensuremath\text{p}}}
\def\rmq{{\ensuremath\text{q}}}
\def\rmr{{\ensuremath\text{r}}}
\def\rmw{{\ensuremath\text{w}}}
\def\rmu{{\ensuremath\text{u}}}
\def\rmv{{\ensuremath\text{v}}}
\def\rms{{\ensuremath\text{s}}}
\def\rmt{{\ensuremath\text{t}}}
\def\rmx{{\ensuremath\text{x}}}
\def\rmy{{\ensuremath\text{y}}}
\def\rmz{{\ensuremath\text{z}}}
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bar bold version
%upper case
%
\def\barbA{{\bar{\ensuremath{\mathbf A}} }}
\def\barbB{{\bar{\ensuremath{\mathbf B}} }}
\def\barbC{{\bar{\ensuremath{\mathbf C}} }}
\def\barbD{{\bar{\ensuremath{\mathbf D}} }}
\def\barbE{{\bar{\ensuremath{\mathbf E}} }}
\def\barbF{{\bar{\ensuremath{\mathbf F}} }}
\def\barbG{{\bar{\ensuremath{\mathbf G}} }}
\def\barbH{{\bar{\ensuremath{\mathbf H}} }}
\def\barbI{{\bar{\ensuremath{\mathbf I}} }}
\def\barbJ{{\bar{\ensuremath{\mathbf J}} }}
\def\barbK{{\bar{\ensuremath{\mathbf K}} }}
\def\barbL{{\bar{\ensuremath{\mathbf L}} }}
\def\barbM{{\bar{\ensuremath{\mathbf M}} }}
\def\barbN{{\bar{\ensuremath{\mathbf N}} }}
\def\barbO{{\bar{\ensuremath{\mathbf O}} }}
\def\barbP{{\bar{\ensuremath{\mathbf P}} }}
\def\barbQ{{\bar{\ensuremath{\mathbf Q}} }}
\def\barbR{{\bar{\ensuremath{\mathbf R}} }}
\def\barbS{{\bar{\ensuremath{\mathbf S}} }}
\def\barbT{{\bar{\ensuremath{\mathbf T}} }}
\def\barbU{{\bar{\ensuremath{\mathbf U}} }}
\def\barbV{{\bar{\ensuremath{\mathbf V}} }}
\def\barbW{{\bar{\ensuremath{\mathbf W}} }}
\def\barbX{{\overline{\bbX}}}
\def\barbY{{\bar{\ensuremath{\mathbf Y}} }}
\def\barbZ{{\bar{\ensuremath{\mathbf Z}} }}
%
%lower case
%
\def\barba{{\bar{\ensuremath{\mathbf a}} }}
\def\barbb{{\bar{\ensuremath{\mathbf b}} }}
\def\barbc{{\bar{\ensuremath{\mathbf c}} }}
\def\barbd{{\bar{\ensuremath{\mathbf d}} }}
\def\barbe{{\bar{\ensuremath{\mathbf e}} }}
\def\barbf{{\bar{\ensuremath{\mathbf f}} }}
\def\barbg{{\bar{\ensuremath{\mathbf g}} }}
\def\barbh{{\bar{\ensuremath{\mathbf h}} }}
\def\barbi{{\bar{\ensuremath{\mathbf i}} }}
\def\barbj{{\bar{\ensuremath{\mathbf j}} }}
\def\barbk{{\bar{\ensuremath{\mathbf k}} }}
\def\barbl{{\bar{\ensuremath{\mathbf l}} }}
\def\barbm{{\bar{\ensuremath{\mathbf m}} }}
\def\barbn{{\bar{\ensuremath{\mathbf n}} }}
\def\barbo{{\bar{\ensuremath{\mathbf o}} }}
\def\barbp{{\bar{\ensuremath{\mathbf p}} }}
\def\barbq{{\bar{\ensuremath{\mathbf q}} }}
\def\barbr{{\bar{\ensuremath{\mathbf r}} }}
\def\barbs{{\bar{\ensuremath{\mathbf s}} }}
\def\barbt{{\bar{\ensuremath{\mathbf t}} }}
\def\barbu{{\bar{\ensuremath{\mathbf u}} }}
\def\barbv{{\bar{\ensuremath{\mathbf v}} }}
\def\barbw{{\bar{\ensuremath{\mathbf w}} }}
\def\barbx{{\bar{\ensuremath{\mathbf x}} }}
\def\barby{{\bar{\ensuremath{\mathbf y}} }}
\def\barbz{{\bar{\ensuremath{\mathbf z}} }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of bar bold bersion
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%hat bold version
%upper case
%
\def\hbA{{\hat{\ensuremath{\mathbf A}} }}
\def\hbB{{\hat{\ensuremath{\mathbf B}} }}
\def\hbC{{\hat{\ensuremath{\mathbf C}} }}
\def\hbD{{\hat{\ensuremath{\mathbf D}} }}
\def\hbE{{\hat{\ensuremath{\mathbf E}} }}
\def\hbF{{\hat{\ensuremath{\mathbf F}} }}
\def\hbG{{\hat{\ensuremath{\mathbf G}} }}
\def\hbH{{\hat{\ensuremath{\mathbf H}} }}
\def\hbI{{\hat{\ensuremath{\mathbf I}} }}
\def\hbJ{{\hat{\ensuremath{\mathbf J}} }}
\def\hbK{{\hat{\ensuremath{\mathbf K}} }}
\def\hbL{{\hat{\ensuremath{\mathbf L}} }}
\def\hbM{{\hat{\ensuremath{\mathbf M}} }}
\def\hbN{{\hat{\ensuremath{\mathbf N}} }}
\def\hbO{{\hat{\ensuremath{\mathbf O}} }}
\def\hbP{{\hat{\ensuremath{\mathbf P}} }}
\def\hbQ{{\hat{\ensuremath{\mathbf Q}} }}
\def\hbR{{\hat{\ensuremath{\mathbf R}} }}
\def\hbS{{\hat{\ensuremath{\mathbf S}} }}
\def\hbT{{\hat{\ensuremath{\mathbf T}} }}
\def\hbU{{\hat{\ensuremath{\mathbf U}} }}
\def\hbV{{\hat{\ensuremath{\mathbf V}} }}
\def\hbW{{\hat{\ensuremath{\mathbf W}} }}
\def\hbX{{\hat{\ensuremath{\mathbf X}} }}
\def\hbY{{\hat{\ensuremath{\mathbf Y}} }}
\def\hbZ{{\hat{\ensuremath{\mathbf Z}} }}
%
%lower case
%
\def\hba{{\hat{\ensuremath{\mathbf a}} }}
\def\hbb{{\hat{\ensuremath{\mathbf b}} }}
\def\hbc{{\hat{\ensuremath{\mathbf c}} }}
\def\hbd{{\hat{\ensuremath{\mathbf d}} }}
\def\hbe{{\hat{\ensuremath{\mathbf e}} }}
\def\hbf{{\hat{\ensuremath{\mathbf f}} }}
\def\hbg{{\hat{\ensuremath{\mathbf g}} }}
\def\hbh{{\hat{\ensuremath{\mathbf h}} }}
\def\hbi{{\hat{\ensuremath{\mathbf i}} }}
\def\hbj{{\hat{\ensuremath{\mathbf j}} }}
\def\hbk{{\hat{\ensuremath{\mathbf k}} }}
\def\hbl{{\hat{\ensuremath{\mathbf l}} }}
\def\hbm{{\hat{\ensuremath{\mathbf m}} }}
\def\hbn{{\hat{\ensuremath{\mathbf n}} }}
\def\hbo{{\hat{\ensuremath{\mathbf o}} }}
\def\hbp{{\hat{\ensuremath{\mathbf p}} }}
\def\hbq{{\hat{\ensuremath{\mathbf q}} }}
\def\hbr{{\hat{\ensuremath{\mathbf r}} }}
\def\hbs{{\hat{\ensuremath{\mathbf s}} }}
\def\hbt{{\hat{\ensuremath{\mathbf t}} }}
\def\hbu{{\hat{\ensuremath{\mathbf u}} }}
\def\hbv{{\hat{\ensuremath{\mathbf v}} }}
\def\hbw{{\hat{\ensuremath{\mathbf w}} }}
\def\hbx{{\hat{\ensuremath{\mathbf x}} }}
\def\hby{{\hat{\ensuremath{\mathbf y}} }}
\def\hbz{{\hat{\ensuremath{\mathbf z}} }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of hat bold  bersion
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tilde bold version
%upper case
%
\def\tbA{{\tilde{\ensuremath{\mathbf A}} }}
\def\tbB{{\tilde{\ensuremath{\mathbf B}} }}
\def\tbC{{\tilde{\ensuremath{\mathbf C}} }}
\def\tbD{{\tilde{\ensuremath{\mathbf D}} }}
\def\tbE{{\tilde{\ensuremath{\mathbf E}} }}
\def\tbF{{\tilde{\ensuremath{\mathbf F}} }}
\def\tbG{{\tilde{\ensuremath{\mathbf G}} }}
\def\tbH{{\tilde{\ensuremath{\mathbf H}} }}
\def\tbI{{\tilde{\ensuremath{\mathbf I}} }}
\def\tbJ{{\tilde{\ensuremath{\mathbf J}} }}
\def\tbK{{\tilde{\ensuremath{\mathbf K}} }}
\def\tbL{{\tilde{\ensuremath{\mathbf L}} }}
\def\tbM{{\tilde{\ensuremath{\mathbf M}} }}
\def\tbN{{\tilde{\ensuremath{\mathbf N}} }}
\def\tbO{{\tilde{\ensuremath{\mathbf O}} }}
\def\tbP{{\tilde{\ensuremath{\mathbf P}} }}
\def\tbQ{{\tilde{\ensuremath{\mathbf Q}} }}
\def\tbR{{\tilde{\ensuremath{\mathbf R}} }}
\def\tbS{{\tilde{\ensuremath{\mathbf S}} }}
\def\tbT{{\tilde{\ensuremath{\mathbf T}} }}
\def\tbU{{\tilde{\ensuremath{\mathbf U}} }}
\def\tbV{{\tilde{\ensuremath{\mathbf V}} }}
\def\tbW{{\tilde{\ensuremath{\mathbf W}} }}
\def\tbX{{\tilde{\ensuremath{\mathbf X}} }}
\def\tbY{{\tilde{\ensuremath{\mathbf Y}} }}
\def\tbZ{{\tilde{\ensuremath{\mathbf Z}} }}
%
%lower case
%
\def\tba{{\tilde{\ensuremath{\mathbf a}} }}
\def\tbb{{\tilde{\ensuremath{\mathbf b}} }}
\def\tbc{{\tilde{\ensuremath{\mathbf c}} }}
\def\tbd{{\tilde{\ensuremath{\mathbf d}} }}
\def\tbe{{\tilde{\ensuremath{\mathbf e}} }}
\def\tbf{{\tilde{\ensuremath{\mathbf f}} }}
\def\tbg{{\tilde{\ensuremath{\mathbf g}} }}
\def\tbh{{\tilde{\ensuremath{\mathbf h}} }}
\def\tbi{{\tilde{\ensuremath{\mathbf i}} }}
\def\tbj{{\tilde{\ensuremath{\mathbf j}} }}
\def\tbk{{\tilde{\ensuremath{\mathbf k}} }}
\def\tbl{{\tilde{\ensuremath{\mathbf l}} }}
\def\tbm{{\tilde{\ensuremath{\mathbf m}} }}
\def\tbn{{\tilde{\ensuremath{\mathbf n}} }}
\def\tbo{{\tilde{\ensuremath{\mathbf o}} }}
\def\tbp{{\tilde{\ensuremath{\mathbf p}} }}
\def\tbq{{\tilde{\ensuremath{\mathbf q}} }}
\def\tbr{{\tilde{\ensuremath{\mathbf r}} }}
\def\tbs{{\tilde{\ensuremath{\mathbf s}} }}
\def\tbt{{\tilde{\ensuremath{\mathbf t}} }}
\def\tbu{{\tilde{\ensuremath{\mathbf u}} }}
\def\tbv{{\tilde{\ensuremath{\mathbf v}} }}
\def\tbw{{\tilde{\ensuremath{\mathbf w}} }}
\def\tbx{{\tilde{\ensuremath{\mathbf x}} }}
\def\tby{{\tilde{\ensuremath{\mathbf y}} }}
\def\tbz{{\tilde{\ensuremath{\mathbf z}} }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of tilde bold  bersion
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bold caligraph
%
\def\bbcalA{\mbox{\boldmath $\mathcal{A}$}}
\def\bbcalB{\mbox{\boldmath $\mathcal{B}$}}
\def\bbcalC{\mbox{\boldmath $\mathcal{C}$}}
\def\bbcalD{\mbox{\boldmath $\mathcal{D}$}}
\def\bbcalE{\mbox{\boldmath $\mathcal{E}$}}
\def\bbcalF{\mbox{\boldmath $\mathcal{F}$}}
\def\bbcalG{\mbox{\boldmath $\mathcal{G}$}}
\def\bbcalH{\mbox{\boldmath $\mathcal{H}$}}
\def\bbcalI{\mbox{\boldmath $\mathcal{I}$}}
\def\bbcalJ{\mbox{\boldmath $\mathcal{J}$}}
\def\bbcalK{\mbox{\boldmath $\mathcal{K}$}}
\def\bbcalL{\mbox{\boldmath $\mathcal{L}$}}
\def\bbcalM{\mbox{\boldmath $\mathcal{M}$}}
\def\bbcalN{\mbox{\boldmath $\mathcal{N}$}}
\def\bbcalO{\mbox{\boldmath $\mathcal{O}$}}
\def\bbcalP{\mbox{\boldmath $\mathcal{P}$}}
\def\bbcalQ{\mbox{\boldmath $\mathcal{Q}$}}
\def\bbcalR{\mbox{\boldmath $\mathcal{R}$}}
\def\bbcalW{\mbox{\boldmath $\mathcal{W}$}}
\def\bbcalU{\mbox{\boldmath $\mathcal{U}$}}
\def\bbcalV{\mbox{\boldmath $\mathcal{V}$}}
\def\bbcalS{\mbox{\boldmath $\mathcal{S}$}}
\def\bbcalT{\mbox{\boldmath $\mathcal{T}$}}
\def\bbcalX{\mbox{\boldmath $\mathcal{X}$}}
\def\bbcalY{\mbox{\boldmath $\mathcal{Y}$}}
\def\bbcalZ{\mbox{\boldmath $\mathcal{Z}$}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of caligraph
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tilde Greek
%
\def\tdupsilon{\tilde\upsilon}
\def\tdalpha{\tilde\alpha}
\def\tbeta{\tilde\beta}
\def\tdgamma{\tilde\gamma}
\def\tddelta{\tilde\delta}
\def\tdepsilon{\tilde\epsilon}
\def\tdvarepsilon{\tilde\varepsilon}
\def\tdzeta{\tilde\zeta}
\def\tdeta{\tilde\eta}
\def\tdtheta{\tilde\theta}
\def\tdvartheta{\tilde\vartheta}

\def\tdiota{\tilde\iota}
\def\tdkappa{\tilde\kappa}
\def\tdlambda{\tilde\lambda}
\def\tdmu{\tilde\mu}
\def\tdnu{\tilde\nu}
\def\tdxi{\tilde\xi}
\def\tdpi{\tilde\pi}
\def\tdrho{\tilde\rho}
\def\tdvarrho{\tilde\varrho}
\def\tdsigma{\tilde\sigma}
\def\tdvarsigma{\tilde\varsigma}
\def\tdtau{\tilde\tau}
\def\tdupsilon{\tilde\upsilon}
\def\tdphi{\tilde\phi}
\def\tdvarphi{\tilde\varphi}
\def\tdchi{\tilde\chi}
\def\tdpsi{\tilde\psi}
\def\tdomega{\tilde\omega}

\def\tdGamma{\tilde\Gamma}
\def\tdDelta{\tilde\Delta}
\def\tdTheta{\tilde\Theta}
\def\tdLambda{\tilde\Lambda}
\def\tdXi{\tilde\Xi}
\def\tdPi{\tilde\Pi}
\def\tdSigma{\tilde\Sigma}
\def\tdUpsilon{\tilde\Upsilon}
\def\tdPhi{\tilde\Phi}
\def\tdPsi{\tilde\Psi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of title  Greek
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bar Greek
%
\def\bbarupsilon{\bar\upsilon}
\def\bbaralpha{\bar\alpha}
\def\bbarbeta{\bar\beta}
\def\bbargamma{\bar\gamma}
\def\bbardelta{\bar\delta}
\def\bbarepsilon{\bar\epsilon}
\def\bbarvarepsilon{\bar\varepsilon}
\def\bbarzeta{\bar\zeta}
\def\bbareta{\bar\eta}
\def\bbartheta{\bar\theta}
\def\bbarvartheta{\bar\vartheta}

\def\bbariota{\bar\iota}
\def\bbarkappa{\bar\kappa}
\def\bbarlambda{\bar\lambda}
\def\bbarmu{\bar\mu}
\def\bbarnu{\bar\nu}
\def\bbarxi{\bar\xi}
\def\bbarpi{\bar\pi}
\def\bbarrho{\bar\rho}
\def\bbarvarrho{\bar\varrho}
\def\bbarvarsigma{\bar\varsigma}
\def\bbarphi{\bar\phi}
\def\bbarvarphi{\bar\varphi}
\def\bbarchi{\bar\chi}
\def\bbarpsi{\bar\psi}
\def\bbaromega{\bar\omega}

\def\bbarGamma{\bar\Gamma}
\def\bbarDelta{\bar\Delta}
\def\bbarTheta{\bar\Theta}
\def\bbarLambda{\bar\Lambda}
\def\bbarXi{\bar\Xi}
\def\bbarPi{\bar\Pi}
\def\bbarSigma{\bar\Sigma}
\def\bbarUpsilon{\bar\Upsilon}
\def\bbarPhi{\bar\Phi}
\def\bbarPsi{\bar\Psi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of bar  Greek
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%begion of check Greek
%
\def\chkupsilon{\check\upsilon}
\def\chkalpha{\check\alpha}
\def\chkbeta{\check\beta}
\def\chkgamma{\check\gamma}
\def\chkdelta{\check\delta}
\def\chkepsilon{\check\epsilon}
\def\chkvarepsilon{\check\varepsilon}
\def\chkzeta{\check\zeta}
\def\chketa{\check\eta}
\def\chktheta{\check\theta}
\def\chkvartheta{\check\vartheta}

\def\chkiota{\check\iota}
\def\chkkappa{\check\kappa}
\def\chklambda{\check\lambda}
\def\chkmu{\check\mu}
\def\chknu{\check\nu}
\def\chkxi{\check\xi}
\def\chkpi{\check\pi}
\def\chkrho{\check\rho}
\def\chkvarrho{\check\varrho}
\def\chksigma{\check\sigma}
\def\chkvarsigma{\check\varsigma}
\def\chktau{\check\tau}
\def\chkupsilon{\check\upsilon}
\def\chkphi{\check\phi}
\def\chkvarphi{\check\varphi}
\def\chkchi{\check\chi}
\def\chkpsi{\check\psi}
\def\chkomega{\check\omega}

\def\chkGamma{\check\Gamma}
\def\chkDelta{\check\Delta}
\def\chkTheta{\check\Theta}
\def\chkLambda{\check\Lambda}
\def\chkXi{\check\Xi}
\def\chkPi{\check\Pi}
\def\chkSigma{\check\Sigma}
\def\chkUpsilon{\check\Upsilon}
\def\chkPhi{\check\Phi}
\def\chkPsi{\check\Psi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of check Greek
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Bold Greek letter
%

\def\bbalpha{\boldsymbol{\alpha}}
\def\bbbeta{\boldsymbol{\beta}}
\def\bbgamma{\boldsymbol{\gamma}}
\def\bbdelta{\boldsymbol{\delta}}
\def\bbepsilon{\boldsymbol{\epsilon}}
\def\bbvarepsilon{\boldsymbol{\varepsilon}}
\def\bbzeta{\boldsymbol{\zeta}}
\def\bbeta{\boldsymbol{\eta}}
\def\bbtheta{\boldsymbol{\theta}}
\def\bbvartheta{\boldsymbol{\vartheta}}
\def \bbtau {\boldsymbol{\tau}}
\def\bbupsilon{\boldsymbol{\upsilon}}
\def\bbiota{\boldsymbol{\iota}}
\def\bbkappa{\boldsymbol{\kappa}}
\def\bblambda{\boldsymbol{\lambda}}
\def\bblam{\boldsymbol{\lambda}}
\def\bbmu{\boldsymbol{\mu}}
\def\bbnu{\boldsymbol{\nu}}
\def\bbxi{\boldsymbol{\xi}}
\def\bbpi{\boldsymbol{\pi}}
\def\bbrho{\boldsymbol{\rho}}
\def\bbvarrho{\boldsymbol{\varrho}}
\def\bbvarsigma{\boldsymbol{\varsigma}}
\def\bbphi{\boldsymbol{\phi}}
\def\bbvarphi{\boldsymbol{\varphi}}
\def\bbchi{\boldsymbol{\chi}}
\def\bbpsi{\boldsymbol{\psi}}
\def\bbomega{\boldsymbol{\omega}}
\def\bbGamma{\boldsymbol{\Gamma}}
\def\bbDelta{\boldsymbol{\Delta}}
\def\bbTheta{\boldsymbol{\Theta}}
\def\bbLambda{\boldsymbol{\Lambda}}
\def\bbXi{\boldsymbol{\Xi}}
\def\bbPi{\boldsymbol{\Pi}}
\def\bbSigma{\boldsymbol{\Sigma}}
\def\bbUpsilon{\boldsymbol{\Upsilon}}
\def\bbPhi{\boldsymbol{\Phi}}
\def\bbPsi{\boldsymbol{\Psi}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of Bold Greek
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bar Bold Greek
%
\def\barbupsilon{\bar\bbupsilon}
\def\barbalpha{\bar\bbalpha}
\def\barbbeta{\bar\bbbeta}
\def\barbgamma{\bar\bbgamma}
\def\barbdelta{\bar\bbdelta}
\def\barbepsilon{\bar\bbepsilon}
\def\barbvarepsilon{\bar\bbvarepsilon}
\def\barbzeta{\bar\bbzeta}
\def\barbeta{\bar\bbeta}
\def\barbtheta{\bar\bbtheta}
\def\barbvartheta{\bar\bbvartheta}

\def\barbiota{\bar\bbiota}
\def\barbkappa{\bar\bbkappa}
\def\barblambda{\bar\bblambda}
\def\barbmu{\bar\bbmu}
\def\barbnu{\bar\bbnu}
\def\barbxi{\bar\bbxi}
\def\barbpi{\bar\bbpi}
\def\barbrho{\bar\bbrho}
\def\barbvarrho{\bar\bbvarrho}
\def\barbvarsigma{\bar\bbvarsigma}
\def\barbphi{\bar\bbphi}
\def\barbvarphi{\bar\bbvarphi}
\def\barbchi{\bar\bbchi}
\def\barbpsi{\bar\bbpsi}
\def\barbomega{\bar\bbomega}

\def\barbGamma{\bar\bbGamma}
\def\barbDelta{\bar\bbDelta}
\def\barbTheta{\bar\bbTheta}
\def\barbLambda{\bar\bbLambda}
\def\barbXi{\bar\bbXi}
\def\barbPi{\bar\bbPi}
\def\barbSigma{\bar\bbSigma}
\def\barbUpsilon{\bar\bbUpsilon}
\def\barbPhi{\bar\bbPhi}
\def\barbPsi{\bar\bbPsi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of bar Bold Greek
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%hat Bold Greek
%
\def\hbupsilon{\hat\bbupsilon}
\def\hbalpha{\hat\bbalpha}
\def\hbbeta{\hat\bbbeta}
\def\hbgamma{\hat\bbgamma}
\def\hbdelta{\hat\bbdelta}
\def\hbepsilon{\hat\bbepsilon}
\def\hbvarepsilon{\hat\bbvarepsilon}
\def\hbzeta{\hat\bbzeta}
\def\hbeta{\hat\bbeta}
\def\hbtheta{\hat\bbtheta}
\def\hbvartheta{\hat\bbvartheta}

\def\hbiota{\hat\bbiota}
\def\hbkappa{\hat\bbkappa}
\def\hblambda{\hat\bblambda}
\def\hbmu{\hat\bbmu}
\def\hbnu{\hat\bbnu}
\def\hbxi{\hat\bbxi}
\def\hbpi{\hat\bbpi}
\def\hbrho{\hat\bbrho}
\def\hbvarrho{\hat\bbvarrho}
\def\hbvarsigma{\hat\bbvarsigma}
\def\hbphi{\hat\bbphi}
\def\hbvarphi{\hat\bbvarphi}
\def\hbchi{\hat\bbchi}
\def\hbpsi{\hat\bbpsi}
\def\hbomega{\hat\bbomega}

\def\hbGamma{\hat\bbGamma}
\def\hbDelta{\hat\bbDelta}
\def\hbTheta{\hat\bbTheta}
\def\hbLambda{\hat\bbLambda}
\def\hbXi{\hat\bbXi}
\def\hbPi{\hat\bbPi}
\def\hbSigma{\hat\bbSigma}
\def\hbUpsilon{\hat\bbUpsilon}
\def\hbPhi{\hat\bbPhi}
\def\hbPsi{\hat\bbPsi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of hat Bold Greek
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tilde Bold Greek
%
\def\tbupsilon{\tilde\bbupsilon}
\def\tbalpha{\tilde\bbalpha}
\def\tbbeta{\tilde\bbbeta}
\def\tbgamma{\tilde\bbgamma}
\def\tbdelta{\tilde\bbdelta}
\def\tbepsilon{\tilde\bbepsilon}
\def\tbvarepsilon{\tilde\bbvarepsilon}
\def\tbzeta{\tilde\bbzeta}
\def\tbeta{\tilde\bbeta}
\def\tbtheta{\tilde\bbtheta}
\def\tbvartheta{\tilde\bbvartheta}

\def\tbiota{\tilde\bbiota}
\def\tbkappa{\tilde\bbkappa}
\def\tblambda{\tilde\bblambda}
\def\tbmu{\tilde\bbmu}
\def\tbnu{\tilde\bbnu}
\def\tbxi{\tilde\bbxi}
\def\tbpi{\tilde\bbpi}
\def\tbrho{\tilde\bbrho}
\def\tbvarrho{\tilde\bbvarrho}
\def\tbvarsigma{\tilde\bbvarsigma}
\def\tbphi{\tilde\bbphi}
\def\tbvarphi{\tilde\bbvarphi}
\def\tbchi{\tilde\bbchi}
\def\tbpsi{\tilde\bbpsi}
\def\tbomega{\tilde\bbomega}

\def\tbGamma{\tilde\bbGamma}
\def\tbDelta{\tilde\bbDelta}
\def\tbTheta{\tilde\bbTheta}
\def\tbLambda{\tilde\bbLambda}
\def\tbXi{\tilde\bbXi}
\def\tbPi{\tilde\bbPi}
\def\tbSigma{\tilde\bbSigma}
\def\tbUpsilon{\tilde\bbUpsilon}
\def\tbPhi{\tilde\bbPhi}
\def\tbPsi{\tilde\bbPsi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of tilde Bold Greek
\def \deltat {\triangle t}
\def \eps    {\epsilon}
\def \lam    {\lambda}
\def \bblam  {\bblambda}
\def \Lam    {\Lambda}
\def \bbLam  {\bbLambda}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%hat greek
%
\def\hhattheta{\hat\theta}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of hat greek

